A Simple Non-i.i.d. Sampling Approach for Efficient Training and Better Generalization

While training on samples drawn from independent and identical distribution has been a de facto paradigm for optimizing image classification networks, humans learn new concepts in an easy-to-hard manner and on the selected examples progressively. Driven by this fact, we investigate the training paradigms where the samples are not drawn from independent and identical distribution. We propose a data sampling strategy, named Drop-and-Refresh (DaR), motivated by the learning behaviors of humans that selectively drop easy samples and refresh them only periodically. We show in our experiments that the proposed DaR strategy can maintain (and in many cases improve) the predictive accuracy even when the training cost is reduced by 15% on various datasets (CIFAR 10, CIFAR 100 and ImageNet) and with different backbone architectures (ResNets, DenseNets and MobileNets). Furthermore and perhaps more importantly, we find the ImageNet pre-trained models using our DaR sampling strategy achieves better transferability for the downstream tasks including object detection (+0.3 AP), instance segmentation (+0.3 AP), scene parsing (+0.5 mIoU) and human pose estimation (+0.6 AP). Our investigation encourages people to rethink the connections between the sampling strategy for training and the transferability of its learned features for pre-training ImageNet models.

==> tables/cifar100_ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]
	%\scriptsize
	\centering
	%\resizebox{1\textwidth}{!}{
	\begin{minipage}[t]{0.5\textwidth}
		\vspace{0pt}
		\centering
		\begin{tabular}{l|c|c}
			Interval & Accuracy & Computation\\
			\hline
			all data & 74.26 & 100\%\\
			baseline & 74.05 & 79\%\\
			\hline
			10 & 72.45 & 63\%\\
% 			15 & 73.07 & 72.8\%\\
			20 & 74.05 & 79\%\\
% 			25 & 73.94 & 83.2\%\\
			30 & 74.25 & 86\%\\
		\end{tabular}
	
	\end{minipage}% <---- don't forget this %
	\begin{minipage}[t]{0.5\textwidth}
		\vspace{0pt}
		\centering	
		\begin{tabular}{l|c|c}
			Active & Accuracy & Computation \\
			\hline
			all data & 74.26 & 100\%\\
			baseline & 74.05 & 79\%\\
			\hline
			40 & 74.43 & 92\%\\ 
			60 & 74.07 & 87\%\\
			no active & 74.05 & 79\%\\
		\end{tabular}
		
	\end{minipage}% <---- don't forget this %
	
	
	\begin{minipage}[b]{.49\textwidth}
		\centering
		(a)
	\end{minipage}
	\begin{minipage}[b]{.49\textwidth}
		\centering
		(b)
	\end{minipage}
	
	\caption{Ablation studies results. Evaluate on CIFAR100 test set. Baseline is ResNet-110 with warm-up epochs=40, interval=20, percentage=0.9, active=$\infty$, reusing all data at $150^{th}$ epochs. (a) Ablation study on number of interval. (b) Ablation study on number of active epochs.}
	\label{tab:cifar100_ablation}

\end{table*}

==> tables/cifar10_ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[t]\setlength{\tabcolsep}{1pt}
	%\scriptsize
	\centering
	%\resizebox{1\textwidth}{!}{
	\begin{minipage}[t]{0.31\textwidth}
		\vspace{0pt}
		\centering
		\begin{tabular}{l|c|c}
			Warm-up & Accuracy & Computation\\
			\hline
			all data & 94.54 & 100\%\\
			baseline & 94.63 & 63\%\\
			\hline
			no warm-up & 93.94 & 53\%\\ 
% 			10 & 93.89\% & 55.5\%\\
			20 & 94.26 & 58\%\\
% 			30 & 94.68\% & 60.4\%\\
			40 & 94.63 & 63\%\\
% 			50 & 94.60\% & 64.8\%\\
			60 & 94.73 & 67\%\\
			70 & 94.80 & 69\%\\
% 			80 & 94.57\% & 70.5\%\\
			90 & 95.04 & 72\%\\
		\end{tabular}
	
	\end{minipage}% <---- don't forget this %
	\begin{minipage}[t]{0.35\textwidth}
		\vspace{0pt}
		\centering	
		\begin{tabular}{l|c|c}
			Interval & Accuracy & Computation \\
			\hline
			all data & 94.54 & 100\%\\
			baseline & 94.63 & 63\%\\
			\hline
			2 & 93.21 & 27\%\\ 
			5 & 93.71 & 44\%\\
			10 & 94.63 & 63\%\\
			15 & 94.63 & 73\%\\
			20 & 94.68 & 79\%\\
			25 & 95.08 & 83\%\\
		\end{tabular}
		
	\end{minipage}	
	\begin{minipage}[t]{.31\textwidth}
		\vspace{0pt}
		\centering		
		\begin{tabular}{l|c|c}
			Percentage & Accuracy & Computation \\
			\hline
			all data & 94.54 & 100\%\\
			baseline & 94.63 & 63\%\\
			\hline
			0.7 & 93.44 & 35\%\\ 
			0.75 & 93.67 & 39\%\\
			0.8 & 94.03 & 45\%\\
			0.85 & 94.45 & 52\%\\
			0.9 & 94.63 & 63\%\\
			0.95 & 94.80 & 78\%\\	
		\end{tabular}
		
	\end{minipage}% <---- don't forget this %
% 	\begin{minipage}[t]{.22\textwidth}
% 		\vspace{0pt}
% 		\begin{tabular}{l|c|c}
% 			Active Epoch & Accuracy & Computation \\
% 			\hline
% 			20 & 94.74\% & 92.0\%\\ 
% 			30 & 94.88\% & 85.4\%\\
% 			40 & 94.53\% & 80.0\%\\
% 			50 & 94.46\% & 75.6\%\\
% 			60 & 94.64\% & 72.1\%\\
% 			$\infty$ & 94.63\% & 62.7\%\\
% 		\end{tabular}
		
% 	\end{minipage}
	%	}	
	
	
	\begin{minipage}[b]{.33\textwidth}
		\centering
		(a)
	\end{minipage}
	\begin{minipage}[b]{.33\textwidth}
		\centering
		(b)
	\end{minipage}
	\begin{minipage}[b]{.33\textwidth}
		\centering
		(c)
	\end{minipage}
% 	\begin{minipage}[b]{.3\textwidth}
% 		\centering
% 		(d)
% 	\end{minipage}

	\begin{minipage}[t]{.3\textwidth}
		\vspace{0pt}
		\begin{tabular}{l|c|c}
			Active & Accuracy & Computation \\
			\hline
			all data & 94.54 & 100\%\\
			baseline & 94.63 & 63\%\\
			\hline
			20 & 94.74 & 92\%\\ 
% 			30 & 94.88\% & 85.4\%\\
% 			40 & 94.53\% & 80.0\%\\
% 			50 & 94.46\% & 75.6\%\\
			60 & 94.64 & 72\%\\
			no active & 94.63 & 63\%\\
		\end{tabular}
		
	\end{minipage}
	%	\resizebox{1\textwidth}{!}{		
	\begin{minipage}[t]{.35\textwidth}
		\vspace{0pt}
		\begin{tabular}{l|c|c} 
			Reusing Data & Accuracy & Computation \\
			\hline
			all data & 94.54 & 100\%\\
			baseline & 94.63 & 63\%\\
			\hline
			\small No reusing & 93.80 & 45\% \\
			\small Reusing at 150 & 94.63 & 63\% \\
			\small Reusing at 150/225 & 94.56 & 73\% \\
		\end{tabular}
		%		\caption{Ablation study on classifier depth.}		
	\end{minipage}
	\begin{minipage}[t]{.3\textwidth}
		\vspace{0pt}
		\begin{tabular}{l|c}
			Strategy & Accuracy \\
			\hline
			\small Ours (63\% computation) & 94.63 \\
			\small Random (63\% computation) & 93.96 \\
			\small All data 63\% epochs & 94.43 \\
			\small 63\% data & 92.21 \\
		\end{tabular}
		%		\caption{Ablation study on base detector.}		
	\end{minipage}
% 	\begin{minipage}[t]{.35\textwidth}		
% 		\vspace{0pt}
% 		\begin{tabular}{l|c}
% 			Model capacity & mAP \\
% 			\hline
% 			Faster w/ Res101 & 79.8 \\
% 			Faster w/ Res152 & 80.3 \\
%             Faster Ensemble & 81.1 \\
% 			Faster w/ Res101+DCR-50 & 82.3\\
% 		\end{tabular}
% 		%		\caption{Ablation study on model capacity.}
% 	\end{minipage}	
	
	\begin{minipage}[b]{.3\textwidth}
		\centering
		(d)
	\end{minipage}
	\begin{minipage}[b]{.35\textwidth}
		\centering
		(e)
	\end{minipage}
	\begin{minipage}[b]{.3\textwidth}
		\centering
		(f)
	\end{minipage}
	%	}
	
	\caption{Ablation studies results. Evaluate on CIFAR10 test set. Baseline is ResNet-110 with warm-up epochs=40, interval=10, percentage=0.9, active=$\infty$, reusing all data at $150^{th}$ epochs. (a) Ablation study on number of warm-up epochs. (b) Ablation study on number of interval. (c) Ablation study on percentage. (d) Ablation study on number of active epochs. (e) Ablation study on strategies of reusing all training data. (f) Ablation study on strategies of training with same amount of computation.}
	\label{tab:cifar10_ablation}

\end{table*}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[t]
% 	%\scriptsize
% 	\centering
% 	%\resizebox{1\textwidth}{!}{
% 	\begin{minipage}[t]{0.33\textwidth}
% 		\vspace{0pt}
% 		\centering
% 		\begin{tabular}{l|c|c}
% 			Warm-up & Accuracy & Computation\\
% 			\hline
% 			all data & 94.54 & 100\%\\
% 			baseline & 94.63 & 63\%\\
% 			\hline
% 			no warm-up & 93.94 & 53\%\\ 
% % 			10 & 93.89\% & 55.5\%\\
% 			20 & 94.26 & 58\%\\
% % 			30 & 94.68\% & 60.4\%\\
% 			40 & 94.63 & 63\%\\
% % 			50 & 94.60\% & 64.8\%\\
% 			60 & 94.73 & 67\%\\
% 			70 & 94.80 & 69\%\\
% % 			80 & 94.57\% & 70.5\%\\
% 			90 & 95.04 & 72\%\\
% 		\end{tabular}
	
% 	\end{minipage}% <---- don't forget this %
% 	\begin{minipage}[t]{0.33\textwidth}
% 		\vspace{0pt}
% 		\centering	
% 		\begin{tabular}{l|c|c}
% 			Interval & Accuracy & Computation \\
% 			\hline
% 			all data & 94.54 & 100\%\\
% 			baseline & 94.63 & 63\%\\
% 			\hline
% 			2 & 93.21 & 27\%\\ 
% 			5 & 93.71 & 44\%\\
% 			10 & 94.63 & 63\%\\
% 			15 & 94.63 & 73\%\\
% 			20 & 94.68 & 79\%\\
% 			25 & 95.08 & 83\%\\
% 		\end{tabular}
		
% 	\end{minipage}	
% 	\begin{minipage}[t]{.33\textwidth}
% 		\vspace{0pt}
% 		\centering		
% 		\begin{tabular}{l|c|c}
% 			Percentage & Accuracy & Computation \\
% 			\hline
% 			all data & 94.54 & 100\%\\
% 			baseline & 94.63 & 63\%\\
% 			\hline
% 			0.7 & 93.44 & 35\%\\ 
% 			0.75 & 93.67 & 39\%\\
% 			0.8 & 94.03 & 45\%\\
% 			0.85 & 94.45 & 52\%\\
% 			0.9 & 94.63 & 63\%\\
% 			0.95 & 94.80 & 78\%\\	
% 		\end{tabular}
		
% 	\end{minipage}% <---- don't forget this %
% % 	\begin{minipage}[t]{.22\textwidth}
% % 		\vspace{0pt}
% % 		\begin{tabular}{l|c|c}
% % 			Active Epoch & Accuracy & Computation \\
% % 			\hline
% % 			20 & 94.74\% & 92.0\%\\ 
% % 			30 & 94.88\% & 85.4\%\\
% % 			40 & 94.53\% & 80.0\%\\
% % 			50 & 94.46\% & 75.6\%\\
% % 			60 & 94.64\% & 72.1\%\\
% % 			$\infty$ & 94.63\% & 62.7\%\\
% % 		\end{tabular}
		
% % 	\end{minipage}
% 	%	}	
	
	
% 	\begin{minipage}[b]{.33\textwidth}
% 		\centering
% 		(a)
% 	\end{minipage}
% 	\begin{minipage}[b]{.33\textwidth}
% 		\centering
% 		(b)
% 	\end{minipage}
% 	\begin{minipage}[b]{.33\textwidth}
% 		\centering
% 		(c)
% 	\end{minipage}
% % 	\begin{minipage}[b]{.3\textwidth}
% % 		\centering
% % 		(d)
% % 	\end{minipage}

% 	\begin{minipage}[t]{.3\textwidth}
% 		\vspace{0pt}
% 		\begin{tabular}{l|c|c}
% 			Active & Accuracy & Computation \\
% 			\hline
% 			all data & 94.54 & 100\%\\
% 			baseline & 94.63 & 63\%\\
% 			\hline
% 			20 & 94.74 & 92\%\\ 
% % 			30 & 94.88\% & 85.4\%\\
% % 			40 & 94.53\% & 80.0\%\\
% % 			50 & 94.46\% & 75.6\%\\
% 			60 & 94.64 & 72\%\\
% 			no active & 94.63 & 63\%\\
% 		\end{tabular}
		
% 	\end{minipage}
% 	%	\resizebox{1\textwidth}{!}{		
% 	\begin{minipage}[t]{.35\textwidth}
% 		\vspace{0pt}
% 		\begin{tabular}{l|c|c} 
% 			Reusing Data & Accuracy & Computation \\
% 			\hline
% 			all data & 94.54 & 100\%\\
% 			baseline & 94.63 & 63\%\\
% 			\hline
% 			\small No reusing & 93.80 & 45\% \\
% 			\small Reusing at 150 & 94.63 & 63\% \\
% 			\small Reusing at 150/225 & 94.56 & 73\% \\
% 		\end{tabular}
% 		%		\caption{Ablation study on classifier depth.}		
% 	\end{minipage}
% 	\begin{minipage}[t]{.3\textwidth}
% 		\vspace{0pt}
% 		\begin{tabular}{l|c}
% 			Strategy & Accuracy \\
% 			\hline
% 			\small Ours (63\% computation) & 94.63 \\
% 			\small Random (63\% computation) & 93.96 \\
% 			\small All data 63\% epochs & 94.43 \\
% 			\small 63\% data & 92.21 \\
% 		\end{tabular}
% 		%		\caption{Ablation study on base detector.}		
% 	\end{minipage}
% % 	\begin{minipage}[t]{.35\textwidth}		
% % 		\vspace{0pt}
% % 		\begin{tabular}{l|c}
% % 			Model capacity & mAP \\
% % 			\hline
% % 			Faster w/ Res101 & 79.8 \\
% % 			Faster w/ Res152 & 80.3 \\
% %             Faster Ensemble & 81.1 \\
% % 			Faster w/ Res101+DCR-50 & 82.3\\
% % 		\end{tabular}
% % 		%		\caption{Ablation study on model capacity.}
% % 	\end{minipage}	
	
% 	\begin{minipage}[b]{.3\textwidth}
% 		\centering
% 		(d)
% 	\end{minipage}
% 	\begin{minipage}[b]{.35\textwidth}
% 		\centering
% 		(e)
% 	\end{minipage}
% 	\begin{minipage}[b]{.3\textwidth}
% 		\centering
% 		(f)
% 	\end{minipage}
% 	%	}
	
% 	\caption{Ablation studies results. Evaluate on CIFAR10 test set. Baseline is ResNet-110 with warm-up epochs=40, interval=10, percentage=0.9, active=$\infty$, reusing all data at $150^{th}$ epochs. (a) Ablation study on number of warm-up epochs. (b) Ablation study on number of interval. (c) Ablation study on percentage. (d) Ablation study on number of active epochs. (e) Ablation study on strategies of reusing all training data. (f) Ablation study on strategies of training with same amount of computation.}
% 	\label{tab:cifar10_ablation}

% \end{table*}

==> tables/cifar_data_redundant.tex <==
\begin{table}[t!]\setlength{\tabcolsep}{1pt}
	\centering
    \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{l|c|c}
    dataset & all data & 79\% comp \\
    \hline
    CIFAR10 (5000 img/cls) & $94.54$ & $84.68_{(+0.14)}$\\
    CIFAR10-5000 (500 img/cls) & $79.20$ & $77.91_{(-1.29)}$\\
	CIFAR100 (500 img/cls) & $74.26$ & $74.05_{(-0.21)}$\\
		\end{tabular}
        }
		\caption{Data redundant in CIFAR datasets.}
        % Comparison with state-of-the-arts reported in recent publications with different backbones.
\label{tab:cifar_data_redundant}
 \vspace{0mm}
\end{table}

% \begin{table}[t!]\setlength{\tabcolsep}{1pt}
% 	\centering
%     \resizebox{0.49\textwidth}{!}{
%     \begin{tabular}{l|c|c|c}
%     dataset & all data & 63\% comp & 79\% comp \\
%     \hline
%     CIFAR10 (5000 img/cls) & $94.54$ & $94.63_{(+0.09)}$ & $84.68_{(+0.14)}$\\
%     CIFAR10-5000 (500 img/cls) & $79.20$ & $77.06_{(-2.14)}$ & $77.91_{(-1.29)}$\\
% 	CIFAR100 (500 img/cls) & $74.26$ & $72.45_{(-1.81)}$ & $74.05_{(-0.21)}$\\
% 		\end{tabular}
%         }
% 		\caption{Data redundant in CIFAR datasets.}
%         % Comparison with state-of-the-arts reported in recent publications with different backbones.
% \label{tab:cifar_data_redundant}
%  \vspace{0mm}
% \end{table}

==> tables/segmentation.tex <==
\begin{table}[h]\setlength{\tabcolsep}{1pt}
	\centering
% 	\tiny
    % \resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|l|c|c}
 Method & Backbone & Pre-train Computation & mIoU \\
        \hline
        
     PSPNet \cite{zhao2017pyramid} & ResNet-50 & 100\% & 74.2 \\
     PSPNet \cite{zhao2017pyramid} & ResNet-50 & 75\% & 74.8 \\
     PSPNet \cite{zhao2017pyramid} & ResNet-50 & 86\% & 74.3 \\
     
    %     \hline
    
    %  PSPNet \cite{zhao2017pyramid} & ResNet-101 & 100\% & - \\
    %  PSPNet \cite{zhao2017pyramid} & ResNet-101 & 74.9\% & - \\
    %  PSPNet \cite{zhao2017pyramid} & ResNet-101 & 86.0\% & - \\
	
		\end{tabular}
        % }
		\caption{\textbf{Cityscapes \texttt{val} semantic segmentation results.}}
        % All detectors use ResNet-101 as backbone and DCR modules use ResNet-152 as base classifier.
        \label{tab:cityscapes}
% \vspace{-2mm}
\end{table}

% \begin{table*}[tb]\setlength{\tabcolsep}{1pt}
% 	\centering
% 	%\tiny
% 	\small
%     \resizebox{1\textwidth}{!}{
% \begin{tabular}{l|l|c|c|ccccccccccccccccccc}
%  Method & Backbone & \makecell[l]{Pre-train\\Computation} & mIoU & \rotatebox{90}{road} & \rotatebox{90}{sidewalk} & \rotatebox{90}{building} & \rotatebox{90}{wall} & \rotatebox{90}{fence} & \rotatebox{90}{pole} & \rotatebox{90}{traffic light} & \rotatebox{90}{traffic sign} & \rotatebox{90}{vegetation} & \rotatebox{90}{terrain} & \rotatebox{90}{sky} & \rotatebox{90}{person} & \rotatebox{90}{rider} & \rotatebox{90}{car} & \rotatebox{90}{truck} & \rotatebox{90}{bus} & \rotatebox{90}{train} & \rotatebox{90}{motorcycle} & \rotatebox{90}{bicycle} \\
%         \hline
       
   
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 100\% & 76.5 & 97.9 & 83.2 & 92.1 & 57.5 & 59.9 & 61.1 & 68.1 & 76.3 & 92.2 & 64.0 & 94.2 & 80.8 & 59.7 & 94.5 & 78.4 & 84.2 & 73.3 & 59.5 & 76.1 \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 75\% & 76.8 & 97.8 & 83.1 & 92.2 & 60.6 & 60.2 & 61.1 & 68.0 & 76.5 & 92.1 & 63.2 & 94.4 & 80.7 & 59.8 & 94.5 & 77.7 & 85.5 & 72.2 & 63.8 & 75.9 \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 86\% & 76.1 & 97.9 & 83.7 & 92.2 & 60.4 & 58.8 & 60.8 & 66.9 & 75.8 & 92.2 & 65.0 & 94.2 & 80.0 & 56.9 & 94.7 & 76.3 & 81.5 & 67.9 & 65.2 & 75.6 \\
%     %   \hline
%       PSPNet \cite{zhao2017pyramid} & ResNet-50 & 100\% & 74.2 & 97.7 & 82.4 & 91.8 & 60.1 & 57.4 & 59.4 & 65.5 & 73.7 & 91.8 & 62.0 & 94.1 & 78.8 & 57.8 & 94.2 & 75.5 & 77.7 & 53.3 & 63.0 & 74.1 \\
%       PSPNet \cite{zhao2017pyramid} & ResNet-50 & 75\% & 74.8 & 97.7 & 82.1 & 91.9 & 57.0 & 56.1 & 59.8 & 65.4 & 72.9 & 91.7 & 62.9 & 94.4 & 79.0 & 58.3 & 94.2 & 67.3 & 82.7 & 72.2 & 61.6 & 73.6 \\
%       PSPNet \cite{zhao2017pyramid} & ResNet-50 & 86\% & 74.3 & 97.6 & 82.1 & 91.8 & 59.4 & 54.6 & 59.3 & 64.6 & 72.7 & 91.7 & 63.2 & 94.3 & 78.9 & 57.1 & 94.0 & 72.8 & 79.2 & 65.0 & 59.5 & 73.7 \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 100\% & 75.6 & 97.8 & 83.3 & 92.2 & 58.5 & 59.8 & 61.7 & 67.8 & 75.8 & 92.1 & 63.2 & 94.3 & 80.5 & 60.4 & 94.4 & 75.0 & 81.5 & 59.2 & 63.3 & 75.5 \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 75\% & 74.8 & 97.8 & 83.3 & 92.2 & 59.8 & 55.9 & 61.0 & 66.9 & 75.0 & 92.1 & 65.3 & 94.4 & 79.6 & 59.0 & 94.4 & 68.5 & 81.4 & 57.5 & 61.9 & 74.6 \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-50 & 86\% & 75.2 & 97.7 & 82.2 & 92.2 & 61.1 & 58.0 & 61.1 & 67.6 & 75.1 & 92.0 & 63.5 & 94.2 & 79.7 & 58.6 & 94.5 & 72.5 & 78.0 & 64.3 & 62.4 & 74.8 \\
      
%     %   \hline
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-101 & 100\% & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-101 & 75\% & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
%     %   PSPNet \cite{zhao2017pyramid} & ResNet-101 & 86\% & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
	
% 		\end{tabular}
%         }
% 		\caption{\textbf{Cityscapes \texttt{val} semantic segmentation results.}}
% \label{tab:cityscapes}
% % \vspace{-8mm}
% \end{table*}
